Precision tests of the AdS/CFT correspondence

This thesis explores various aspects of precision holography through the study of supersymmetric quantum field theories and their gravitational duals. In addition to previously published work, it contains a systematic investigation of one-loop logarithmic corrections in a broad class of $AdS_4$ Kaluza-Klein supergravities, including previously unpublished results. The theories under consideration arise from compactifications of eleven-dimensional, massive type IIA, and type IIB supergravity. By examining a large set of $AdS_4$ vacua connected by holographic renormalization group (RG) flows in $SO(8)$ and $ISO(7)$ gauged supergravities, I find that the coefficients of the logarithmic corrections agree at the UV and IR fixed points of all flows considered. This observation motivates a conjecture of their universal invariance under holographic RG flows. For compactifications of massive type IIA and type IIB supergravity where independent field-theory results are available, I further demonstrate exact holographic agreement.

==> adsphd-master/chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}

\ldots

\instructionsabstract


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> adsphd-master/chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}

\ldots


\instructionsabstract

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> adsphd-master/chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{This is curriculum}\label{ch:curriculum}

\ldots

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> adsphd-master/chapters/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}

\subsection{Image on the cover page}

If you want to place an image on the cover of the dissertation, you can add
the code underneath to the template (check with your promotor whether this is
allowed).

\paragraph{Include image:}
Search for the \texttt{\textbackslash frontcoverheaderXII} command in
the \texttt{adsphd.cls} file and add the following lines:
\begin{verbatim}
   \begin{textblock*}{56mm}(10mm+#1,15mm)
   \includegraphics[width=56mm,height=20mm]{image/filename}
   \end{textblock*}
\end{verbatim}
Where 56mm is the width, 20mm the height, 10mm the x-location and 15mm the
y-location.

\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> adsphd-master/chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Preface}                                  \label{ch:preface}

\ldots

\instructionspreface


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> adsphd-master/mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother


==> chapters/abstract/abstract.tex <==
% !TeX root = ../../thesis.tex
\chapter{Abstract}                                 \label{ch:abstract}


% \instructionsabstract

	The AdS/CFT correspondence, or holographic duality, relates quantum field theories with quantum gravity in one dimension higher. In this thesis, we study precision holography in various examples, using tools from strongly-coupled quantum field theories and supergravity.
	
	After reviewing the AdS/CFT correspondence in the introductory chapter \ref{ch:introduction}, in chapter \ref{ch:ads4log} we study 4d gauged supergravity theories that can be uplifted to 10d or 11d supergravity backgrounds. Motivated by results in the holographically dual 3d field theories, we examine the logarithmic corrections to the gravitational on-shell action and black hole entropy for a number of theories on different backgrounds, both supersymmetric and non-supersymmetric. By comparing our new results with the field theories' results, we have confirmed precision holography and found new Swampland constraints on the gravity theories.
	
	In chapter \ref{ch:etheory}, we study a specific 4d $\cN = 2$ superconformal gauge theory called the $\bf E$ theory. This theory is closely related to the $\cN = 4$ super Yang-Mills theory and has  a holographic description in terms of type IIB supergravity on a $\mathbb{Z}_2$ orientifold of AdS$_5 \times S^5$. With novel high precision numerics, we evaluate the partition function on $S^4$, extremal correlators, and vacuum expectation values of Wilson loops with general 't Hooft coupling in the planar limit. Based on these numerics, we arrive at closed-form formulas in the strong coupling expansion. Our results match the literature on type IIB supergravity.
	
	In chapter \ref{ch:ads8}, we study the Hawking-Page phase transition between two asymptotically locally AdS$_8$ families of backgrounds, which are analogs of NUT and Bolt in the 4d counterpart. The backgrounds are parametrized by a squashing parameter of the asymptotic boundary, which is a squashed seven-sphere. Surprisingly, we observe the absence of the Hawking-Page transition, giving a prediction for the dual non-supersymmetric field theory. We also calculate and compare the free energies as a function of the squashing parameter in conformally coupled scalar, free fermion, and the holographic theory.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/abstractnl/abstractnl.tex <==
% !TeX root = ../../thesis.tex
\chapter{Beknopte samenvatting}

% Version translated by chatGPT:

%De AdS/CFT-correspondentie, of holografische dualiteit, verbindt kwantumveldtheorieën met kwantumzwaartekracht in een hogere dimensie. In deze thesis bestuderen we precieze holografie in verschillende voorbeelden, met behulp van tools uit sterk gekoppelde kwantumveldtheorieën en superzwaartekracht.

%Na de AdS/CFT-correspondentie te hebben besproken in het inleidende hoofdstuk \ref{ch:introduction}, bestuderen we in hoofdstuk \ref{ch:ads4log} 4d geschaalde superzwaartekrachttheorieën die kunnen worden opgeheven naar 10d of 11d superzwaartekrachtachtergronden. Gemotiveerd door resultaten in de holografisch duale 3d veldtheorieën, onderzoeken we de logaritmische correcties op de gravitationele on-shell actie en zwarte gat entropie voor een aantal theorieën op verschillende achtergronden, zowel supersymmetrisch als niet-supersymmetrisch. Door onze nieuwe resultaten te vergelijken met de veldtheorieën resultaten, hebben we precieze holografie bevestigd en nieuwe Swampland-constraints gevonden op de zwaartekrachttheorieën.

%In hoofdstuk \ref{ch:etheory}, bestuderen we een specifieke 4d $\cN = 2$ superconforme gauge-theorie genaamd de $\bf E$-theorie. Deze theorie is nauw verwant aan de $\cN = 4$ super Yang-Mills-theorie en heeft een holografische beschrijving in termen van type IIB superzwaartekracht op een $\mathbb{Z}_2$ orientifold van AdS$_5 \times S^5$. Met behulp van nieuwe hoge-precisie numerieke methoden, evalueren we de partitie functie op $S^4$, extremale correlatoren en vacuum expectation values van Wilson lussen met algemene 't Hooft koppeling in de vlakke limiet. Gebaseerd op deze numerieke methoden, komen we tot gesloten formules in de sterke koppeling uitbreiding. Onze resultaten komen overeen met de literatuur over type IIB superzwaartekracht.

%In hoofdstuk \ref{ch:ads8}, bestuderen we de Hawking-Page faseovergang tussen twee asymptotisch lokaal AdS$_8$ families van achtergronden, die analogen zijn van NUT en Bolt in het 4d tegenhanger. De achtergronden worden geparametriseerd door een squash-parameter van de asymptotische grens, die een gesquashte zevensfeer is. Verrassend genoeg observeren we de afwezigheid van de Hawking-Page overgang, wat een voorspelling geeft voor de duale niet-supersymmetrische veldtheorie. We berekenen en vergelijken ook de vrije energieën als functie van de squash-parameter in conform gekoppelde scalar, vrije fermion en de holografische theorie.

% \instructionsabstract

% Version corrected by Annelien:

De AdS/CFT-correspondentie, of holografische dualiteit, verbindt kwantumveldtheorieën met kwantumzwaartekracht in een hogere dimensie. In deze thesis bestuderen we precisie-holografie in verschillende voorbeelden, met behulp van tools uit sterk gekoppelde kwantumveldtheorieën en superzwaartekracht.

Na de AdS/CFT-correspondentie te hebben besproken in het inleidende hoofdstuk \ref{ch:introduction}, bestuderen we in hoofdstuk \ref{ch:ads4log} de 4d geijkte superzwaartekrachttheorieën die kunnen worden geuplift naar 10d of 11d superzwaartekrachtachtergronden. Gemotiveerd door resultaten in de holografisch duale 3d veldtheorieën, onderzoeken we de logaritmische correcties op de gravitationele on-shell actie en de entropie van een zwart gat voor een aantal theorieën op verschillende achtergronden, zowel supersymmetrisch als niet-supersymmetrisch. Door onze nieuwe resultaten te vergelijken met de veldtheorie-resultaten, hebben we precisie-holografie bevestigd en nieuwe Swampland-constraints gevonden op de zwaartekrachttheorieën.

In hoofdstuk \ref{ch:etheory}, bestuderen we een specifieke 4d $\cN = 2$ superconforme ijktheorie genaamd de $\bf E$-theorie. Deze theorie is nauw verwant aan de $\cN = 4$ super Yang-Mills-theorie en heeft een holografische beschrijving in termen van type IIB superzwaartekracht op een $\mathbb{Z}_2$ orientifold van AdS$_5 \times S^5$. Met behulp van nieuwe hoge-precisie numerieke methoden, evalueren we de partitie functie op $S^4$, extremale correlatoren en vacuum verwachtingswaarden van Wilson lussen met algemene 't Hooft koppeling in de vlakke limiet. Gebaseerd op deze numerieke methoden, komen we tot gesloten formules in de uitbreiding naar sterke koppeling. Onze resultaten komen overeen met de literatuur over type IIB superzwaartekracht.

In hoofdstuk \ref{ch:ads8}, bestuderen we de Hawking-Page faseovergang tussen twee asymptotisch lokale AdS$_8$ families van achtergronden, die analoog zijn aan NUT en Bolt in de 4d tegenhanger. De achtergronden worden geparametriseerd door een squash-parameter van de asymptotische grens, die een gesquashte zevensfeer is. Verrassend genoeg observeren we de afwezigheid van de Hawking-Page overgang, wat een voorspelling geeft voor de duale niet-supersymmetrische veldtheorie. We berekenen en vergelijken ook de vrije energieën als functie van de squash-parameter in conform gekoppelde scalar, vrije fermion en de holografische theorie.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/conclusion/conclusion.tex <==
% !TeX root = ../../thesis.tex
\chapter{Conclusion and outlook}\label{ch:conclusion}



%\instructionsconclusions

	In this thesis we mainly do two things. The first is to test precision holography. The second is to take advantage of the precision AdS/CFT correspondence to have a better understanding on both the quantum gravity and the strongly-coupled quantum field theories. 
	
	Chapter \ref{ch:ads4log} mainly uses supergravity techniques to reproduce the subleading terms in the dual field theories, which is a non-trivial test of precision holography at quantum level. At the same time, using AdS/CFT, the observation in field theory results that partitions functions and correlators are independent of continuous parameters imposes strong constraints on the bulk theories, and especially may be used to disprove some theories in supergravity with scale separation.
	
	Chapter \ref{ch:etheory} uses field theory techniques to evaluate several BPS observables at strong coupling in the large $N$ limit for the first time, this gives non-trivial predictions on scattering of Kaluza-Klein modes in the dual type IIB supergravity. At the same time, partial results in the gravity side are consistent to ours, which is a non-trivial precision test of holography.
	
	Chapter \ref{ch:ads8} studies the phases and the analogue of Hawking-page phase transition in the Euclidean Einstein gravity for a novel asymptotically AdS$_8$ background. The phase space unexpectedly indicates an absence of any phase transition, which gives a non-trivial prediction on its dual field theory, which is not understood because of the lack of supersymmetry. As a bottom-up model of holography, we compare the partition functions among the conformal scalar, the free fermion, and the holographic theories.
	
	As discussed in the end of each chapters, there are numerous directions of further studies of these stories. Here we highlight some of them as valuable topics to be explored in the future.
	
	\begin{itemize}
		\item The methods we have employed can be generalized to study logarithmic corrections to path integrals in de Sitter space, see \cite{Anninos:2020hfj,Bobev:2022lcc} for some recent explorations in this direction. It is important to develop this topic further and calculate both logarithmic corrections to the entropy of empty de Sitter space as well as to the entropy of asymptotically de Sitter black holes.
		
		\item Supersymmetric localization has proven to be an efficient method for the calculation of path integrals in supersymmetric theories. It may be possible to use localization calculations in gauged supergravity as an efficient method to compute the Euclidean gravitational path integral and access the logarithmic corrections discussed above. This has been explored in \cite{Dabholkar:2014wpa,Hristov:2018lod,Hristov:2019xku,Hristov:2021zai} and it is important to address the subtleties and open questions that accompany this method. We hope that the results presented in this work will prove helpful in this regard. To this end, it is encouraging to note the fact that the 4d KK supergravity regularization discussed in Section~\ref{sec:log-conj} yields the same $\chi \log (L^2/G_N)$ structure of the logarithmic correction as the one found in \cite{Hristov:2021zai} using supergravity localization and index theorems.
		
		\item The methods we used in this work can be applied to logarithmic corrections of AdS path integrals in other space-time dimensions. It will be particularly interesting to perform such an analysis for even-dimensional asymptotically AdS backgrounds since then there are non-trivial local contributions to the logarithmic corrections and it should be possible to deduce constraints on gravitational theories in AdS as we did in Section~\ref{sec:Kundera}.
		
		\item In Section~\ref{sec:Kundera} we presented general constraints on the spectrum of light excitations around a given AdS$_4$ vacuum arising from a UV-complete quantum gravitational theory. It is important to understand whether these constraints are obeyed by the many known AdS$_4$ vacua in string and M-theory. This is of particular interest in the context of scale-separated AdS vacua where these new constraints can either rule out some a priori admissible backgrounds, or point to exotic features in the holographically dual 3d CFTs. It will also be interesting to explore the interplay between the constraints on the matter fields presented in Section~\ref{sec:Kundera} and the species bound discussed in the work of Dvali \cite{Dvali:2007hz}. Finally, we note that in many examples discussed in Section~\ref{sec:KK}, we found that the total heat kernel coefficients of two AdS$_4$ solutions connected by a gravitational domain wall are the same. It is important to understand whether this is a general feature of AdS vacua connected by domain walls. If such a property is generally true it can be used in conjunction with the constraints from Section~\ref{sec:Kundera} to derive even stronger consistency conditions on gravitational theories in AdS.
		
		\item New BPS observables in the superconformal $\bf E$-theory have been studied using similar matrix models that we discuss, such as correlators of Wilson loops \cite{Pini:2023lyo}, correlation function between one single-trace scalar operator and a circular Wilson loop \cite{Pini:2023svd}, integrated two-point functions with a Wilson loop \cite{Billo:2023ncz}, integrated four-point functions \cite{Billo:2023kak}. It would be very interesting to study the limit of our algorithm and to study the strongly coupled limit of these observables for which analytic methods are not powerful enough.
		
		\item There're several aspects of the SO(5)$\times$SO(3) symmetric AlAdS$_8$ space that are interesting to explore. We have not identified the detailed behavior of the renormalized free energy when the squashing parameter approaches the special value $\lambda_* = \frac{1}{\sqrt{5}}$, which requires higher numerical precision. It would be interesting to see whether there is an oscillating behavior around the conically singular solution as observed in \cite{Aharony:2019vgs}. Besides numerics, this special limit can also be studied from the NUT side analytically following the metric perturbation method as in \cite{Aharony:2019vgs}.
		
		\item Given the lack of superconformal field theories in $d = 7$ \cite{Nahm:1977tg, Shnider:1988wh}, there have been many explorations on non-conformal supersymmetric Yang-Mills theory living on seven manifolds, which can be constructed as the worldvolume theory of the D6 branes in the Euclidean type IIA$^*$ theory. \cite{Prins:2018hjc} With supersymmetries, localization calculations can be done to extract information about the free energy and the Wilson loops expectation values. \cite{Bobev:2019bvq} With background fluxes turned on, we expect the free energy to be different from our case, but it would be interesting to compare our results and illustrate the difference.

	\end{itemize}
	
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/curriculum/curriculum.tex <==
% !TeX root = ../../thesis.tex
\chapter{This is curriculum}\label{ch:curriculum}

\ldots

\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/introduction/introduction.tex <==
% !TeX root = ../../thesis.tex
\chapter{Introduction} \label{ch:introduction}

% \instructionsintroduction

	Strongly coupled field theories and quantum gravity are two very intriguing topics in high energy physics. The AdS/CFT correspondence, a mysterious feature of quantum gravity, has been shown to act as an extremely useful and powerful tool to connect them. The goal of the thesis is to study precision AdS/CFT using tools in supergravity and quantum field theories. Besides, the correspondence itself also gives new predictions on both sides. As an introduction, we will start with questions relevant in the thesis that are also interesting to a wider audience, discussing their relations with the AdS/CFT correspondence. In section \ref{sec:symmetry}, we introduce the main field theory tools we use in the thesis, namely superconformal symmetry and supersymmetric localisation. In section \ref{sec:adscft}, we motivate and introduce the AdS/CFT correspondence. The structure of the thesis is given in the end of this chapter.
	
	\subsection*{The black hole entropy }
	
	The first question is related to black hole entropy. For almost 50 years, people have known that the black holes behave like thermal systems characterized by a non-vanishing entropy proportional to the area of the event horizon. \cite{Bardeen:1973gs} Although the area law can be found purely from the classical physics (general relativity), the coefficient is harder to obtain and turns out to include the Planck's constant: \cite{Bekenstein:1973ur, Hawking:1975vcx, Gibbons:1976ue} 
	\begin{equation}
			S_{\rm BH} = \frac{A}{4 l_P^2},\quad l_P = \sqrt{\frac{G_N \hbar}{c^3}},
	\end{equation}
	where $A$ is the area of the horizon. So in order to know what are the microstates attributed to the (very large)\footnote{For example, the entropy of the black hole with one solar mass is around $10^{18}$ times that of the sun. \cite{Bekenstein:1973ur}. } entropy, we need more information from quantum gravity.
	
	There are different perspectives to study the black hole entropy. From the ``top-down'' perspective, people start from the string theory, which is regarded as a consistent quantum theory of gravity. In string theory, some black-holes could be constructed out of objects such as D-branes, NS5 branes, and fundamental strings: in specific brane constructions, the microstates can be parametrized by their momentum quanta explicitly, whose number can be calculated which reproduces the Bekenstein-Hawking formula in the leading order of large charge. \cite{Strominger:1996sh, Mathur:2005ai} There are also insights coming from AdS/CFT correspondence, where the mircostates of asymptotically AdS supersymmetric extremal black holes\footnote{They are also called BPS black holes which are the ground states in the Hilbert space of quantum gravity. } can be evaluated by supersymmetric partition functions of the dual field theories. Various field theory results in the literature are summarized in Table \ref{tab:CFT-log}, which motivate our study in chapter \ref{ch:ads4log}. In this thesis, instead of relying on the AdS/CFT correspondence, we start with a classical background\footnote{By classical it means the background solves the classical equations of motion, with no quantum effects included. } in gauged supergravity theories, and consider quantum fluctuations of all the fields to the partition function. The Legendre transformation of the partition function gives the enetropy. \cite{Mandal:2010cj, Banerjee:2011jp, Bhattacharyya:2012wz} In chapter \ref{ch:ads4log} of the thesis, we study the one-loop quantum corrections to the classical\footnote{Here the word ``classical'' means that the Bekenstein-Hawking entropy is evaluated from the classical background. } Bekenstein-Hawking. 
	
	\subsection*{Strongly coupled field theories}
	In field theories, the weak-coupling behavior can be studied through Feynman diagrams in a systematic way. However, the strong-coupling regime is also important and interesting for us. There are situations where a strong coupling necessarily appears. For example, because of the asymptotic freedom, the non-Abelian gauge theories (or Yang-Mills theories) are strongly-coupled in the low-energy regime, resulting in the quark-confinement. So a strong-coupling is involved if we were to study the confinement-deconfinement phase transition in QCD. Another example is in AdS/CFT correspondence, where the field theory becomes strongly-coupled if we want to suppress the high-derivative corrections in the corresponding gravity theory, which is necessary for the precision holography since we don't know the full tower of high-derivative corrections of string theory.
	
	After so many years of research, there are already many powerful non-pertbative techniques to study quantum field theories. For example, the introduction of conformal symmetry and supersymmetry, large $N$ expansion, and integrability. The development of computing power and more efficient algorithms is also helpful, which prompted the lattice gauge theories. The AdS/CFT correspondence also plays an important role for studying holographic field theories, because it maps a strongly-coupled field theory to a weak-coupling gravity theory. At the same time, the AdS/CFT correspondence maps a strongly-coupled gravity to a weakly-coupled field theory, so it also probes the unknown regimes of quantum gravity.
	
	\subsection*{The path integral of quantum gravity}
	Path integral is a natural way to do quantization. Let's start with the gravitational path integral in Lorentzian signature:
	\begin{equation} \label{eq:QGPI}
	Z_{\rm grav}^L = \int \cD g_{\mu\nu} \cD\phi e^{ i \frac{1}{\hbar} I^L[g_{\mu\nu}, \phi]},
	\end{equation}
	with $I^L[g_{\mu\nu}, \phi]$ the Einstein-Hilbert action plus possible matter contents. A useful operation in field theory path integral is the Wick rotation, which people also apply to study the gravitational path integral:
	\begin{equation}
	Z_{\rm grav}^E = \int \cD g_{\mu\nu} \cD\phi e^{ - \frac{1}{\hbar} I^E[g_{\mu\nu}, \phi]}.
	\end{equation}
	The advantage of the Wick rotation is that the WKB approximation in which $\hbar \rightarrow 0$ performs better. This can be understood as follows. In the WKB limit, the path integral can be approximated by saddle-points, or stationary phases, which are backgrounds such that the classical equations of motion are solved. Under the WKB approximation, the path integrals are dominated by these saddles, up to small corrections in $\hbar$:
	\begin{equation}
	\begin{aligned}
			Z_{\rm grav}^L & = \sum_{g^{\rm cl}_{\mu\nu}, \phi^{\rm cl}} e^{i\frac{1}{\hbar} I^L[g^{\rm cl}_{\mu\nu}, \phi^{\rm cl}]} \left( 1 + \sum_{n=1} \alpha_n(i\hbar)^n \right) ,\\ 
			Z_{\rm grav}^E & =  \sum_{g^{\rm cl}_{\mu\nu}, \phi^{\rm cl}} e^{-\frac{1}{\hbar} I^E[g^{\rm cl}_{\mu\nu}, \phi^{\rm cl}]} \left( 1 + \sum_{n=1} \alpha_n(-\hbar)^n \right),
	\end{aligned}
	\end{equation}
	where the sum in front of each line is over all classical saddles $g^{\rm cl}_{\mu\nu}, \phi^{\rm cl}$ that solve the equations of motion. It's not hard to see that there are two advantages to use the Euclidean path integral. First, let us ignore the perturbative corrections and focus on the leading term contribution given by the action. In the Euclidean case, only one (or coincidentally a few) saddle(s) with the lowest action will dominate, with the others exponentially suppressed going like $e^{-\Delta I^E /\hbar}$. While in the Lorentzian case, each saddle contributes an order 1 number with different phases. Secondly, by comparing the terms perturbative in $\hbar$, it's not hard to see that the corrections in terms of $(-\hbar)$ cancel with each other and give a smaller total correction. So the Euclidean path integral has smaller perturbative corrections as well.
	
	To sum up, the gravitational path integral \eqref{eq:QGPI} is evaluated by the Euclidean saddles in the classical limit $\hbar \rightarrow 0$: \cite{Gibbons:1976ue}
	\begin{equation} \label{eq:GibbonsHawking}
	Z_{\rm grav} \simeq \sum_{i} e^{-\frac{1}{\hbar} I[g^{(i)}_{\mu\nu}, \phi^{(i)}]},
	\end{equation}
	where the sum is over saddle-points, namely backgrounds which satisfy the classical equations of motion of the path integral with given boundary conditions. This Euclidean prescription will play a central role in our studies in various gravity theories. This is accompanied by the fact that we also have a better control on the field theories in Euclidean signature. As we know from the study of quantum field theories, the observables suffer from UV and IR divergences. The former appears due to the high-energy modes, and the latter is a result of the space-time being unbounded. As we will see, the supersymmetric localisation automatically solves the UV divergences by reducing the full path integral to an integration of zero modes or fixed locus. To solve the IR divergences, we need to put the theory on a compact manifold, so we need to use the Euclidean signature in the field theory as well to get rid of the unbounded Lorentzian time coordinate.
	
	The Gibbons-Hawking integral allows us to approximate the path integral by a sum over Euclidean saddles, but we don't know whether the classical background with the lowest action is really a minimum or only a saddle\footnote{This ``saddle'' means that the action $I^E$ may decrease further upon a small off-shell deformation of the background. }, especially because the Einstein-Hilbert action is not bounded from below. \cite{Gibbons:1978ac} Yet in practice, the saddle-point approximation is the most natural thing to do, thus, it is a non-trivial but important task to make sure that the Gibbons-Hawking prescription gives the correct gravitational path integral in the classical limit. One may need alternative ways to study or even define the gravitational path integral. The AdS/CFT correspondence provides a good way to check the Gibbons-Hawking path integral. According to the AdS/CFT correspondence, the gravity partition function $Z_{\rm grav}$ is fully captured by the dual field theory. If it's possible to evaluate the partition function purely from the field theory, we can explicitly check whether the saddle-point approximation is correct in the classical limit. Doing this on the field theory side usually involves strong couplings, but it can be made possible with the techniques of superconformal symmetry and supersymmetric localisation to be introduced in section \ref{sec:symmetry}.
	
	\subsection*{Phase space of AdS spacetime}
	According to the Gibbons-Hawking prescription, in the classical limit, the gravitational path integral is dominated by one or several saddle-points that has the lowest action. With the same boundary conditions, there might exist several competing saddle points. When one changes parameters that determine the boundary condition, such as the temperature or the squashing parameter, the dominant saddle may change. 
	
	One of the examples is given by Hawking-Page phase transition in asymptotically Euclidean AdS space. We know that black holes evaporate, the smaller a black hole is, the faster it evaporates, so the black holes are not stable in asymptotically flat space. But in asymptotically AdS space, massive fields are effectively trapped and can't propagate to the spatial infinity. As a result, the black holes can be in equillibrium with the radiation and become stable. Between the two competing phases, AdS black hole phase and thermal AdS phase, there exists a critical temperature where the dominant phase changes. It is an interesting question to study the structure of the phase space of the gravitational path integral in the classical limit, such as what are the possible phases, when do they dominate, and what's the order of the phase transition.
	
	$ $
	
	In order to study these questions discussed above, we should first have proper tools. So before going to the more specific questions in later chapters, we shall have a brief review on the main tools. In the following section, I will introduce the superconformal symmetry in Euclidean signature and supersymmetric localisation which are helpful for studying the strongly-coupled field theories. After that, I will introduce the AdS/CFT correspondence, including its motivation, a constructive example, and its implications.

	\section{Aspects of symmetry} \label{sec:symmetry}
	
	Symmetry plays an important role in modern physics. In classical physics, we already know that a global symmetry gives a conserved charge, when the number of the symmetry is large, the system becomes ``integrable'' and the evolution is largely constrained. We will introduce conformal symmetry and supersymmetry, both of which are cornerstones of the AdS/CFT correspondence and will play an important role throughout the whole thesis.
	
		\subsection{Conformal symmetry and supersymmetry}
	As discussed before, in this thesis, we use the Euclidean signature for the field theories. For a generic relativistic field theory, the set of symmetry includes translations $P_\mu$ and Lorentzian transformations $M_{\mu\nu}$, where $\mu = 0,1,\cdots, d$ is the space-time label. Combing them gives the Poincar\'e group, which preserves the (proper) distance:
	\begin{equation}
		\frac{\partial x'^{\mu}}{\partial x^\nu} = R^\mu_{\ \nu},\quad R^TR = I_{d\times d}.
	\end{equation}
	Critical systems in nature, such as the critical systems, enjoy extra scaling symmetry: $x \rightarrow \lambda x$. The most general set of symmetry transformations that preserves the angle but not the distance is called conformal symmetry\footnote{The scaling symmetry itself doesn't imply the full conformal symmetry, namely the special conformal transformation $K_\mu$, see discussion in \cite{Nakayama:2013is}. }, i.e.,
	\begin{equation}
		\frac{\partial x'^{\mu}}{\partial x^\nu} = \Omega(x)^2 R^\mu_{\ \nu}, \quad R^TR = I_{d\times d},
	\end{equation}
	which include the Poincar\'e group, the dilatations generator $D$ that generates the scaling symmetry, and the special conformal symmetry $K_\mu$. The conformal symmetry turns out to be very powerful. Field theories that accommodate conformal symmetry are called conformal field theories. For eigenstates $\cO_i$ of the dilatations generator with eigenvalues $\Delta_i$, the two-point and three-point functions are determined up to constant factors:
	\begin{equation}
	\begin{aligned}
		\langle \cO_i(x) \cO_j(y) \rangle & \sim \frac{\delta_{ij}}{|x-y|^{\Delta_1 + \Delta_2}}, \\
		\langle \cO_i(x) \cO_j(y) \cO_k(z) \rangle & \sim \frac{\lambda_{ijk}}{|x-y|^{\Delta_1 + \Delta_2 - \Delta_3}|y-z|^{\Delta_2 + \Delta_3 - \Delta_1}|z-x|^{\Delta_3 + \Delta_1 - \Delta_2}}. \\
	\end{aligned}
	\end{equation}
	The conformal symmetry is in fact more powerful. Through the program of conformal boostrap \cite{Hartman:2022zik, Poland:2022qrs}, one may determine accurately the data of the field theory, such as the conformal dimensions\footnote{In Euclidean signature, we usually do the radial quantization, where the ``constant time slices'' are taken to be the surfaces with constant radii. In this quantization, the dilatations generator $D$ plays the role of the Hamiltonian which generates the time evolution, so the conformal dimensions are sometimes also called the ``energies''. } $\Delta_i$ and OPE coefficients $\lambda_{ijk}$ for the operators. Though being interesting and powerful, the conformal boostrap will not be the focus of this thesis.
	
	Now we introduce the supersymmetry \cite{Golfand:1971iw, Wess:1974tw, Haag:1974qh} to conformal field theories, which are generated by operators $Q$ that transform bosonic states into fermionic states and vice versa:
	\begin{equation}
		[Q, B] = F,\quad \{Q, F\} = B.
	\end{equation}
	Since the operation of the supercharge $Q$ changes the spin by $1/2$, if we require the maximal spin within a quantum field theory not to exceed $1$, there will be a maximal number of total supersymmetry. In fact, the representations of all possible super-conformal symmetry in different dimensions have been worked out, which only exists in $d\le 6$, \cite{Nahm:1977tg, Cordova:2016emh} and we will be interested in $d = 3, 4$ in this work. In each superconformal multiplet, the bosons and fermions are organized such that their total degrees of freedom are equal.
	
	Supersymmetric gauge theories play an important role in the AdS/CFT correspondence, as they encode aspects of space-time in quantum gravity. The landscape of studies on SCFTs (superconformal field theories) is immense and is still under great progress nowadays \cite{Argyres:2022mnu}, powerful tools such as supersymmetric localization \cite{Pestun:2016zxk}, integrability \cite{Beisert:2010jr}, and superconformal bootstrap \cite{Hartman:2022zik, Poland:2022qrs}, among many others, enable us to get a deeper understanding of the field theories, and thus have a great impact on holography. According to the AdS/CFT correspondence, fields in the gravity theories are mapped to fields in the superconformal field theories, which are organized into superconformal multiplets in accordance with the amount of supercharges. 

	
	\subsection{ A brief overview of supersymmetric localisation}
		
	My work uses supersymmetric localization to study supersymmetric field theories. Mathematically, the supersymmetry generators $Q$'s are similar to the equivariant differential forms. As a result, the domain of the path integral is reduced to a subset of the full configuration space called the BPS locus, where the fields are annihilated by $Q$. In favourable situations, the field theory path integrals that evaluate BPS observables, such as the partition functions, correlators, and expectation values of the Wilson loops, are reduced to finite dimensional integrals. 
	
	Let's first look at the idea of ``localisation''. For an integral over a manifold $\cM$, if the integrand satisfies some simplifying properties, for example it is a total derivative, then we only need to evaluate the integral on $\partial \cM$. If $\partial \cM$ happens to be a set of points, the full integral localizes to the points. This is the most na\"ive example of localisation.
	
	What we actually do is more involved, and the localised points are not simply on boundary of the domain. For an example \cite{Cremonesi:2013twh} which catches some of the salient features of localisation, we consider the following integral on $S^2$ parametrized by a real number $t$:
	\begin{equation}
		Z(t) = \int_0^{2\pi} d\phi \int_0^{\pi} \sin\theta d\theta\ e^{it f(\theta, \phi)}, \quad f (\theta, \phi) = \cos \theta.
	\end{equation}
	In the large $t$ limit, one may consider a stationary-phase approximation, under which the integral is reduced to the sum of Gaussian integrals with quadratic fluctuations about each stationary point $x^*$:
	\begin{equation}
		Z(t) = \frac{2\pi i}{t} \sum_{x^*} (-i)^{\lambda(x^*)} \frac{e^{itf(x^*)}}{\sqrt{\det(g^{-1} H_f(x^*)) }} + O(t)^{-2},
			\end{equation}
	where $H_f$ is the Hessian of $f$, which for the standard metric $ds^2 = d\theta^2 + \sin^2\theta d\phi^2$ gives:
	\begin{equation}
		H_f = \nabla_i \nabla_j f(x) = \diag(-\cos\theta, \cos\theta).
	\end{equation}
	Since our function $f = \cos \theta$ is nothing but the height function, whose stationary points $x^*$ are the north and south poles. Plugging in the values, we get the leading order under the stationary phase approximation:
	\begin{equation}
		Z = \frac{2\pi i}{t} \left[ (-i) \frac{e^{it}}{\sqrt{-1}} + (-i) \frac{e^{-it}}{\sqrt{-1}} \right] + O(t)^{-2}.
	\end{equation}
	At the same time, we can do the integral directly to get the exact answer:
	\begin{equation}
		Z(t) = 2\pi \int_{-1}^1 d(\cos\theta) e^{it\cos\theta} = \frac{2\pi i}{t} \left(-e^{it} + e^{-it} \right).
	\end{equation}
	By comparing the stationary phase approximation and the exact result, we see that up to the correct choices of branches for the square root function, the stationary phase approximation gives an exact answer. The reason is that function $f$ is invariant under the U(1) isometry of the two-sphere rotating along the $z$-axis. For this special case, the integral is reduced to the fixed points of the U(1) isometry, which is exactly the stationary points of $f$. This is an example of the Duistermaat-Heckman localisation formula \cite{Duistermaat:1982vw} based on fixed points of isometries, which is in turn an example of a more general equivariant localisation formula. \cite{Witten:1982im, Atiyah:1984px}
	
	Supersymmetric localization \cite{Witten:1988ze, Witten:1991zz, Pestun:2007rz} is an analogue of equivariant localisation \footnote{There is a more detailed map between quantities in equivariant localisation and quantities in supersymmetric localisation, as introduced in \cite{Cremonesi:2013twh}. We will not get into these details. }, which aims at evaluating the expectation values of BPS observables $\cO_{\rm BPS}$:
	\begin{equation}
	\langle \cO_{\rm BPS} \rangle = \int \cD X \cO_{\rm BPS} e^{-S[X]},\quad \cQ \cO_{\rm BPS} = 0,
	\end{equation}
	where $\cQ$ is a supersymmetric generator and it squares to a bosonic generator, $\cQ^2 = B$, which can be a linear combination of spacetime symmetries, global symmetries, and the gauge symmetry. We have the analog of Stokes' theorem in supersymmetric field theories, which dictates that the $\cQ$-exact operators don't contribute to the expectation value:
	\begin{equation}
	\langle \cQ \cO \rangle = \int \cD X (\cQ \cO) e^{-S[X]} = \int \cD X \cQ \left( \cO e^{-S[X]} \right) = 0,
	\end{equation}
	assuming that there are no boundary contributions or anomalies. Now we consider deforming the integrand by adding a $\cQ$-exact term $\cQ \cP[X]$ with an additional constraint on the fermionic term such that $B \cP[X] = 0$. Then we can check that the deformed path integral is independent of the deformation parameter $t$:
	\begin{equation}
	\begin{aligned}
	& \frac{d}{dt} \int \cD X \cO_{\rm BPS} e^{-S[X] - t \cQ \cP[X]} = - \int \cD X (\cQ \cP[X]) \cO_{\rm BPS} e^{-S[X] - t \cQ \cP[X]} \\
	&\quad = -  \int \cD X \cQ \left( \cP[X] \cO_{\rm BPS} e^{-S[X] - t \cQ \cP[X]}  \right) = 0,
	\end{aligned}
	\end{equation}
	where we used the invariance of $\cP$ under the bosonic transformation $B = \cQ^2$ and the invariance of $\cO_{\rm BPS}e^{-S[X]}$ under $\cQ$. Because of the independence of $t$, we can evaluate the path integral in the limit $t\rightarrow \infty$, where the saddle-point approximation becomes exact. The saddle points are located at the BPS locus $\cF_{\rm BPS}$, which are fixed points of $\cQ$ in the full field space, which is given by:
	\begin{equation}
	\cF_{\rm BPS} \equiv \{ X = X_0 | {\rm fermions} = 0,\ \cQ ({\rm fermions}) = 0 \}.
	\end{equation}
	Under the saddle-point approximation, the classical value combined with the 1-loop fluctuations over the BPS locus gives the exact path integral over the infinite-dimensional field theory space. Consider the following fluctuation:
	\begin{equation}
	X = X_0 + \frac{1}{\sqrt{t}} \delta X,
	\end{equation}
	where $X_0$ denotes the BPS configuration. When taking the large $t$ limit, we take the BPS value of the original action $S[X_0]$ and choose the form of $\cP[X]$ such that the deformation $\cQ \cP[X]$ vanishes at the BPS locus and only the quadratic fluctuations survive:
	\begin{equation}
	S[X] + t \cQ \cP[X] \rightarrow S[X_0] + \frac{1}{2} \int \frac{\delta^2 (\cQ \cP) }{\delta X^2} \Big|_{X = X_0} (\delta X)^2 + O(1/\sqrt{t}).
	\end{equation}
	So the BPS observable reduces to:
	\begin{equation} \label{eq:LocalizedPathIntegral}
	\langle \cO_{\rm BPS} \rangle = \int \cD X_0 \cO_{\rm BPS}\Big|_{X = X_0} e^{-S[X_0]} \frac{1}{{\rm SDet}\left[ \frac{\delta^2 (\cQ \cP[X_0]) }{\delta X_0^2} \right]}.
	\end{equation}
	In favorable cases with suitable choices of deformation $\cQ \cP[X]$, the integral over the BPS locus can be expressed as a finite-dimensional integral, making the formidable evaluation possible. One typical choice of deforming action is:
	\begin{equation}
	\cP = \sum (\cQ \Psi)^\dagger \Psi + \Psi^\dagger (\cQ \Psi),\quad \cQ \cP = \sum (\cQ \Psi)^\dagger (\cQ \Psi),
	\end{equation}
	where we sum over all the fermions. The resulting integral is in general an $N$-dimensional one, which is still very complicated for an arbitrary $N$. Other techniques based on matrix model, integrability, complex analysis, or even statistical mechanics will be used to study these integrals. In fact, the main technical improvement of chapter \ref{ch:etheory} is devoted to evaluating the matrix model by a combination of numerics and strong/weak-coupling expansion.
	
	Application of localization principle to quantum field theories has been long restricted to topological field theories with scalar supersymmetry. A major breakthrough was made by Pestun \cite{Pestun:2007rz} who constructed $\cN = 2$ supersymmetric gauge theories on $S^4$ and derived a closed formula for partition function as well as expectation values of certain Wilson loops. We will introduce relevant results in 4d $\cN = 2$ SCFTs in section \ref{sec:N2summary}. Soon after Pestun, using supersymmetric localization, partition functions of 3d $\mathcal{N}=2$ SCFTs on various compact manifolds can be reduced to matrix models. We will introduce some 3d backgrounds with more details in section \ref{sec:SCFT}.

\section{The AdS/CFT correspondence} \label{sec:adscft}

    \subsection{The holographic principle}

Classical works on black hole thermodynamics show that the black-hole entropy satisfies the area law instead of the volume law. \cite{Bardeen:1973gs} One consequence is that in any theory with gravity, the entropy enclosed by a surface $\Sigma$ has an upper bound given by its surface:
\begin{equation} \label{eq:BekensteinBound}
S[\Sigma] \le S_{\rm BH}[\Sigma] \equiv \frac{A[\Sigma]}{4l_P^2},
\end{equation}
where $A[\Sigma]$ denotes the area of the surface and $l_P$ is the Planck length in 4d. The argument can be sketched as follows. Imagine some matters enclosed by $\Sigma$ with $S > S_{\rm BH}$, we can throw in some matter until a black hole is formed\footnote{We will not discuss why will the horizon organize itself on $\Sigma$. Instead, we only discuss systems which will form a horizon on $\Sigma$. As a result, in the present discussion, the Bekenstein bound only applies to a special set of surfaces where a horizon can be formed on it. }, whose entropy is given by $S_{\rm BH}$ indicated above. However, with more matter thrown in, the entropy must increase, this contradicts our assumption above. Thus we have the Bekenstein bound \eqref{eq:BekensteinBound}.

Given the area-law entropic upper bound for a theory with gravity, one may propose that all the degrees of freedom within a theory of gravity can be mapped to a boundary theory without gravity\footnote{We are making this assumption otherwise the chain will never end. But there are discussions on ``double holography'' where people project the gravity on a codimensional-one brane which has its own boundary. \cite{Bueno:2022log} } in one dimension lower. This is similar to how a hologram works, so the proposal above is called the ``holographic principle''. \cite{tHooft:1993dmi, Susskind:1994vu} To have a taste of this principle, one may consider a lattice model of space-time where degrees of freedom are fixed on the lattice, whose lattice length is given by the Planck length. For a generic configuration of this model, the energy enclosed in a closed surface $\Sigma$, which is proportional to its volume, will exceed that of a black hole, so a black hole will form and take place the original configuration. As a result, most of the lattice model configurations are excluded by the black hole formation, and the reduced number of configurations satisfies the area law.

The appearance of the Planck's constant in the Bekenstein bound strongly indicates that quantum effects play an important role in the holographic principle. Similar to Bohr's formula of hydrogen energy levels for quantum mechanics, the holographic principle acts as the touchstone for theories of quantum gravity. Since string theory is a candidate for quantum gravity, which is the first theory able to give the correct number of black hole microstates \cite{Strominger:1996sh}, it is expected to obey this principle as well. In fact, string theory (and M theory) not only satisfies this principle but also provides a highly valuable playground based on explicit constructions of the quantum gravity theory and its corresponding quantum field theories, which is the AdS/CFT correspondence.

\subsection{Gauge theories and strings}

In some sense, it is not completely unexpected that the string theory is connected with gauge theories, because the original motivation of string theory is to describe the strong interaction, where the confined color flux lines connecting two quarks within a meson behave like a string. \cite{Polyakov:1997tj} Namely, the elementary excitations in the confining QCD are not particles but strings that are formed from the flux lines of color fields. This serves as the first picture of gauge/string relation. The stretchable string model gives the correct relation between mass and angular momentum observed in particle physics, i.e., 
\begin{equation}
J = \alpha' M^2 + \alpha(0).
\end{equation}
Although the string theory turns out not a good theory for strong interaction, the fact that the open string represents gauge theories on its endpoints persists. The string theory also contains graviton modes on closed strings, the interactions between open and closed strings suggest a relation between the gauge and gravity theories. 

Another perspective that finally leads to gauge/string correspondence is the large $N$ limit of 4d gauge theory with gauge group SU($N$). \cite{tHooft:1973alw} The gauge fields transform under the adjoint representation of the gauge group, using the fact that
\begin{equation}
{\bf Ad} \oplus {\bf 1} = {\bf N} \otimes \bar{\bf N},
\end{equation}
in the large $N$ limit, we can approximate the gauge field to transform under the bifundamental representation, which introduces the double-line notation for its Feynman diagram representation with two oriented lines carrying fundamental indices. We introduce the 't Hooft coupling $\lambda \equiv g_{\rm YM}^2 N$, so the Lagrangian can be written as
\begin{equation}
\cL = \frac{1}{g_{\rm YM}^2} (\partial A \partial A + A^2 \partial A + A^4) = \frac{N}{\lambda}(\cdots).
\end{equation}
Thus, we have:
\begin{itemize}
	\item For each propagator, there is a factor of $\lambda/N$.
	
	\item For each vertex, there is a factor $N/\lambda$.
	
	\item For each loop, there is a factor $N$ because of the summation of the fundamental index over the closed single-line loop.
\end{itemize}
For simplicity, we focus on the vacuum diagrams of gauge fields with $V$ vertices, $E$ propagators, and $F$ loops, the factor gives:
\begin{equation}
\left( \frac{N}{\lambda}\right)^V \left( \frac{\lambda}{N}\right)^E N^F = \lambda^{E-V} N^{V-E+F}.
\end{equation}
Notice that $V - E + F = \chi$ which is the Euler characteristic. We can fill all the single-line closed loops in a vacuum diagram to make it a two-dimensional closed surface, whose genus $\mathfrak{g}$ is given by $\chi = 2 - 2\mathfrak{g}$. Thus in the large $N$ limit, the partition function can be written as a genus expansion:
\begin{equation}
\log Z_{\rm gauge} = \sum_{\mathfrak{g} = 0} N^{2-2\mathfrak{g}} F_{\mathfrak{g}}(\lambda).
\end{equation}
This is reminiscent of the loop expansion in string theory:
\begin{equation}
\log Z_{\rm string} = \sum_{\mathfrak{g} = 0} (g_s)^{2\mathfrak{g} - 2} \tilde{F}(\alpha'),
\end{equation}
where $g_s$ is the string coupling. The similarity makes 't Hooft conjecture a duality between gauge theory and string theory:
\begin{equation}
g_s \propto 1/N.
\end{equation}
This picture works well in the large $N$ regime, where the diagrams are dominated by those with genus $0$, or the ``planar diagrams''. Another simplification is that in the large $N$ regime, the dual string picture is expected to be weakly coupled, allowing perturbative calculations. 

\subsection{The example of D3 branes}

The proposal of the AdS/CFT correspondence \cite{Maldacena:1997re} is motivated by the previous works on branes and relations to gauge field theories living on the branes. The correspondence suggests that the gravity theory and the field theory correspond to each other in a much larger parameter space in a stronger sense, even at the quantum level. To have a taste of how it works, we take the example of a stack of $N$ D3-branes in type IIB supergravity with $N$ large. One can view the low energy limit of this system from different perspectives, which lead to different descriptions of the same system.

The first perspective on the stack of branes is to look at the brane action. In the low energy limit, we have: \cite{Aharony:1999ti}
\begin{equation}
I = I_{\rm open} + I_{\rm closed} + I_{\rm int}.
\end{equation}
The open-string excitations $I_{\rm open}$ describe the 4d $\cN = 4$ super Yang-Mills theory on the world volume. The closed-string excitations $I_{\rm closed}$ describe a supergravity theory in which the branes are located. $I_{\rm int}$ is the interaction between the two sectors. When taking the limit where $\alpha' \rightarrow 0$, the all the interactions are suppressed, and the open and closed-string sectors get decoupled. The higher derivative stringy corrections to $I_{\rm closed}$ and $I_{\rm open}$ are also suppressed under this limit. As a result, in the limit $\alpha' \rightarrow 0$, the stack of branes is described by the 4d $\cN = 4$ SYM living on the brane with a free supergravity in the 10d space.

The second perspective is from the supergravity point of view, where the metric backreacted by a large stack of D3-branes is given by: \cite{Horowitz:1991cd}
\begin{equation}
\begin{aligned}
ds^2 &= \left( 1 + \frac{R^4}{r^4}\right)^{-1/2}(-dt^2 + d\vec{x}^2) + \left( 1 + \frac{R^4}{r^4}\right)^{1/2}(dr^2 + r^2 d\Omega_5^2),\\
 R^4 &= 4\pi g_s \alpha'^2 N,
\end{aligned}
\end{equation}
with $R$ the AdS length scale. Similarly, we focus on the low-energy modes in this space. Some low-energy modes are massless particles propagating in the bulk, and the others come from excitations living in the near-horizon region, whose energies are suppressed because of the gravitational red-shift. Work on scattering with branes \cite{Klebanov:1997kc, Gubser:1997yh} shows that these two modes decouple in the low energy limit.

Now, we focus on the near-horizon modes and we look at the near-horizon limit $r \ll R$, the geometry will become AdS$_5\times S^5$:
\begin{equation} \label{eq:AdSCoordinate}
ds^2 = \frac{r^2}{R^2} (-dt^2 + d\vec{x}^2 ) + R^2 \frac{dr^2}{r^2} + R^2 d\Omega_5^2.
\end{equation}
To sum up, in the perspective of supergravity, the stack of branes is described by a full quantum gravity theory in AdS$_5\times S^5$ and the massless modes of supergravity propagating in the bulk. 

By comparing these two perspectives, we can see that the excitations in the near horizon region of the branes are described by two completely different theories, i.e., the $\cN = 4$ super Yang-Mills field theory versus quantum gravity excitations in AdS$_5\times S^5$. A careful study show the following dictionary between parameters on both sides:
%    \begin{equation}
%        \frac{4\pi i}{g_{\rm YM}^2} + \frac{\theta}{2\pi} = \frac{i}{g_s} + C_0,\quad g_{\rm YM}^2 N = \frac{R^4}{(\alpha')^2} .
%    \end{equation}
    \begin{equation} \label{eq:dictionaryAdS5CFT4}
       g_{\rm YM}^2 = 4\pi g_s ,\quad \lambda = \frac{R^4}{(\alpha')^2}.
    \end{equation}
Remember that $\lambda = g_{\rm YM}^2 N$ is the 't Hooft coupling. Since the $\cN = 4$ super Yang-Mills and quantum gravity in AdS$_5\times S^5$ both describe the stack of D3 branes, it is conjectured that these two theories are equivalent. Moreover, comparisons on protected observables on both sides can be done, which suggest the validity of the correpsondence beyond the limits. Schematically, this dictates: \cite{Gubser:1998bc, Witten:1998qj}
\begin{equation}
Z[{\rm Type\ IIB\ superstring\ in\ AdS_5\times}S^5] = Z[\cN = 4\ {\rm SYM}],
\end{equation}
including all higher-derivative and quantum corrections. The left-hand side of the equality is the gravitational partition function, and the right-hand side is the generating function of correlators in the field theory. The boundary condition for the gravitational partition function is such that the asymptotic values of the fields are identified with the sources coupling to the fields in the field theory. This is why we always refer to the boundary field theory and the bulk gravitational theory. Based on similar arguments, the same duality occurs from different brane configurations in superstring or M theories, where can make the same comparison between the two perspectives and make a more general statement: \cite{Gubser:1998bc, Witten:1998qj}
\begin{equation}
Z[{\rm Type\ IIA/IIB/M\ theories\ in\ AdS}_d\times M_{D-d}] = Z[{\rm worldvolume\ SCFT}],
\end{equation}
where $D = 10$ or $11$, and $M_{D-d}$ is the compact internal space, which depends on the background in which we put the branes. However, the emergence of AdS space-time isn't necessarily associated to the near-horizon region of branes. \cite{Polyakov:1997tj, Polyakov:2000ti, Polyakov:2000jg} One can understand the extra dimension in the bulk as the energy scale of the boundary. The conformal symmetry of the AdS space \eqref{eq:AdSCoordinate} goes like: 
\begin{equation}
	r\rightarrow \alpha r, \quad x_i\rightarrow x_i/\alpha,
\end{equation} 
	with $x_i$ the space-time coordinate on the boundary field theory. By taking $\alpha$ large, we are approaching the boundary; but at the same time, the probe has a smaller spatial extension, and thus probes higher energy. This is referred to as the UV/IR relation in the duality. \cite{Susskind:1998dq, Peet:1998wn} By pushing $\lambda$ towards infinity, we will encounter both the IR divergence in the bulk because of the divergent volume of the AdS space, and the UV divergence in the boundary field theory. So a cutoff together with counter terms have to be introduced to cure the IR divergence in the bulk. \cite{Henningson:1998gx, deHaro:2000vlm}
	
	Given the above considerations, the most general AdS/CFT correspondence can be independent of brane constructions or even a UV-complete gravity theory:
	\begin{equation}
		Z[{\rm Any\ gravity\ theory\ in\ AdS}] = Z[{\rm A\ certain\ CFT\ on\ }\partial {\rm AdS}].
	\end{equation}
	Some of the examples exist in bottom-up constructions, which are less understood compared to the top-down ones. Especially, without a brane construction, for generic cases it is unclear what field theory is the correct one. These perspectives can be justified by thinking of the boundary field theory as defining the gravity theory in the bulk. In fact, because of technical simplicity, the bottom up holography also provides a lot of new insights to the AdS/CFT correspondence, for example, the dual between JT gravity and SYK model \cite{Stanford:2019vob}, the dual between 2d ensemble averaged field theories and 3d Euclidean wormholes \cite{Cotler:2020ugk}. 
	
	A precision test of the AdS/CFT is in general hard. That's because the two sides of the correspondence are simplified in different regions. Let's take the $\cN=4$ SYM/AdS$_5\times S^5$ correspondence as an example, where the dictionary is \eqref{eq:dictionaryAdS5CFT4}. For the field theory to be perturbative, one expects the effective expansion to be small, i.e.,
	\begin{equation}
	g_{\rm YM}^2 N = \lambda \ll 1,
	\end{equation}
	where an extra factor $N$ is included which comes from summing over the fundamental indices in the loops. (see, e.g., \cite{Balasubramanian:1997kd}) On the other hand, for the gravity theory to be approximated by GR, one wishes that the curvature radius $R$ to be large compared to the string length $l_s = (\alpha')^{1/2}$:
	\begin{equation}
	\frac{R^4}{l_s^4} = \frac{R^4}{(\alpha')^2} = \lambda \gg 1.
	\end{equation}
	In my thesis, I mainly consider a classical action in the bulk gravity theory, and use the powerful tools we introduced in the last section to study the strongly coupled field theories.

	\subsection{Implications of AdS/CFT}
		After more than 20 years since its appearance, the AdS/CFT correspondence has been proven to be very valuable in both quantum gravity and quantum field theories. On one hand, with more results available from both sides beyond the leading order, the correspondence gains more evidence both classically and with quantum corrections; on the other hand, one can take advantage of this correspondence and give non-trivial predictions both in field theory and in quantum gravity.
	
	The topics of my thesis involve the following top-down constructions of AdS/CFT:
	\begin{itemize}
		\item Correspondence between 3d Chern-Simon SCFT arising from M2 branes and 4d gauged supergravity with 10d or 11d upliftings. (Chapter \ref{ch:ads4log})
		
		\item The correspondence between the 4d $\cN = 2$ superconformal {\bf E}-theory and type IIB supergravity in AdS$_5\times S^5/\mathbb{Z}_2$. (Chapter \ref{ch:etheory})   
	\end{itemize}
	
	Let us summarize the relations among the different topics discussed in this section, shown in Fig. \ref{fig:QGStringAdSCFT}. Originally, the string theory as a model of the strong interaction naturally motivates the string/gauge correspondence. The correspondence persists in quantum gravity when the string theory is realised as a theory describing quantum gravity. Holographic principle is motivated by the Bekenstein bound and is a very important feature of quantum gravity. The AdS/CFT is a good example of holography in quantum gravity, and is also a good example of the string/gauge correspondence.  
	
	%\begin{equation}
	%{\rm Quantum}\ {\rm Gravity} \quad \supset \quad 
	%\left\{ \begin{aligned}
	%& {\rm Holography}\\
	%& {\rm Gauge/String}\ {\rm Duality} 
	%\end{aligned} \right. \quad \supset \quad {\rm AdS/CFT}.
	%\end{equation}
	\tikzstyle{G} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black, fill=violet!10]
	\tikzstyle{arrow} = [thick,->,>=stealth]
	\begin{figure}
		\centering
		\begin{tikzpicture}[node distance=3cm]
		
		%%nodes
		\node (QG) [G, text width=3cm,minimum height=1cm,minimum width=1cm, xshift=-5cm] {Quantum Gravity};
		
		\node (StringGauge) [G, text width=3cm,minimum height=1cm,minimum width=2cm, xshift=0cm, yshift=2cm] {String/Gauge Correspondence};
		
		\node (Holography) [G, text width=3cm,minimum height=1cm,minimum width=2cm, xshift=0cm , yshift=-2cm] {Holography};
		
		\node (AdSCFT) [G, text width=3cm,minimum height=1cm,minimum width=2cm, xshift=5cm] {AdS/CFT\\ Correspondence};
		
		%%draw
		\draw[-latex, very thick, shorten >=15pt,shorten <=15pt, ->]    (StringGauge) to (QG);
		
		\draw[-latex, very thick, shorten >=15pt,shorten <=15pt, ->]    (QG) to (Holography);
		
		\draw[-latex, very thick, shorten >=15pt,shorten <=15pt, ->]    (StringGauge) to (AdSCFT);
		
		\draw[-latex, very thick, shorten >=15pt,shorten <=15pt, ->]    (Holography) to (AdSCFT);
		
		\end{tikzpicture}
		\caption{\rm The relation between quantum gravity, the string/gauge correspondence, holographic principle, and the AdS/CFT correspondence. } \label{fig:QGStringAdSCFT}
	\end{figure}
	
	We talked about the correspondence between partition functions above, but we can also insert operators on both sides. For local operator insertions, we get a correspondence between correlation functions on the boundary and S-matrix in the bulk. \cite{Witten:1998qj} For non-local insertions, we have correspondence between expectation value of a Wilson loop on the boundary and surface of string worldsheet in the bulk. \cite{Maldacena:1998im} The entanglement entropy on the boundary is captured by the extremal surface in the bulk. \cite{Ryu:2006bv, Hubeny:2007xt} So the field theory is indeed encoding lots of information about the bulk. In chapter \ref{ch:etheory}, we study various observables in holographic superconformal $\bf E$ theory and give non-trivial predictions to corresponding quantities in the dual supergravity.
	
	So how would the field theory encode the Hawking-Page transition? For the field theory to contain enough degrees of freedom corresponding to black holes in the bulk, we need to take the large $N$ limit. Because of the distinction in topologies between the black-hole and thermal AdS phases, the wrappings of Wilson loops are different between them. The two different configurations of Wilson loops give $O(N)^0$ and $O(N)^2$ large $N$ behavior of the free energy that correspond to the confined and deconfined phases in the Yang-Mills gauge theory. \cite{Witten:1998qj, Witten:1998zw} In chapter \ref{ch:ads8}, we study the Hawking-Page transition in Einstein gravity between two families of asymptotically locally AdS$_8$ spaces. 
	
	As discussed above, the correspondence has a mixing between UV and IR on the two sides, and especially the radial direction of the AdS space is related to an energy scale of the boundary field theory. This is the idea behind the holographic renormalization group flow \cite{deBoer:1999tgo, deBoer:2000cz}, where the bulk theory interpolates two different field theories on two sides which are related by renormalisation group flow. This bulk discription provides a probe to study these renormalisation group flows, not only on the two sides but along the flow itself. Our setup in chapter \ref{ch:ads8} can be understood as such a holographic flow, which is induced by a relevant deformation sourced by the stress-energy tensor.
	
	\section{Structure of the thesis}
	
	In the thesis, we will study the questions introduced in the beginning with more details and try to give a partial answer. The study is mainly motivated by and based on the AdS/CFT correspondence, making use of the tools we introduced above. The contents will be divided into three parts, based on my publications \cite{Bobev:2023dwx}, \cite{Bobev:2022grff}, and \cite{Zhang:2022nim} together with unpublished results. My publication \cite{Cano:2022ord} is not included in the thesis.
	
	In chapter \ref{ch:ads4log} based on \cite{Bobev:2023dwx}, we study the logarithmic corrections to various CFT partition functions in the context of the AdS$_4$/CFT$_3$ correspondence for theories arising on the worldvolume of M2-branes. We utilize four-dimensional gauged supergravity and heat kernel methods and present general expressions for the logarithmic corrections to the gravitational on-shell action and black hole entropy for a number of different supergravity backgrounds. We outline several subtle features of these calculations and contrast them with a similar analysis of logarithmic corrections performed directly in the eleven-dimensional uplift of a given four-dimensional supergravity background. We find results consistent with AdS/CFT provided that the infinite sum over KK modes on the internal space is regularized in a specific manner. This analysis leads to an explicit expression for the logarithmic correction to the Bekenstein-Hawking entropy of large Kerr-Newmann and Reissner-Nordström black holes in AdS$_4$. Our results also have important implications for effective field theory coupled to gravity in AdS$_4$ and for the existence of scale-separated AdS$_4$ vacua in string theory, which come in the form of new constraints on the field content and mass spectrum of matter fields.
	
	Based on unpublished results, we study the logarithmic corrections within gauged supergravity theories that are connected by RG flows. It turns out that any two theories connected by an RG flow give identical logarithmic correction.
	
	In chapter \ref{ch:etheory} based on \cite{Bobev:2022grff}, we study correlation functions of local operators and Wilson loop expectation values in the planar limit of a 4d $\mathcal{N}=2$ superconformal $\SU(N)$ YM theory with hypermultiplets in the symmetric and antisymmetric representations of the gauge group. This so called $\mathbf{E}$ theory is closely related to $\mathcal{N}=4$ SYM and has a holographic description in terms of a $\mathbb{Z}_2$ orientifold of AdS$_5\times S^5$. Using recent matrix model results based on supersymmetric localization we develop efficient numerical methods to calculate two- and three-point functions of certain single trace operators as well as 1/2-BPS Wilson loop expectation values as a function of the 't Hooft coupling $\lambda$. We use our numerical results to arrive at simple analytic expressions for these correlators valid up to sixth order in the $\lambda^{-1/2}$ strong coupling expansion. These results provide explicit field theory predictions for the $\alpha'$ corrections to the supergravity approximation of type IIB string theory on the AdS$_5\times S^5/\mathbb{Z}_2$ orientifold.
	
	In chapter \ref{ch:ads8} based on \cite{Zhang:2022nim}, we study a bottom-up model which involves an asymptotically locally AdS$_8$ analog of the Taub-NUT solution. This chapter presents two main results. First, we study the renormalized free energies of Euclidean Einstein gravity in asymptotically AdS$_8$ and various field theories on a squashed seven sphere. In the gravity theory, we demonstrate the absence of the Hawking-Page transition, while in the field theory, we focus on the O($N$) vector model and the massless free fermion model. The conformal symmetry governs the universal behaviors of the free energies for small and large squashings, which we confirm numerically and analytically. Second, we evaluate the second-order derivative of CFT free energy with respect to the squashing parameter, finding universal results that hold for generic conformal field theories. We examine two different squashings, one with an SU(2) bundle, which is the primary focus of this chapter, and another with a U(1) bundle, where our results align with the conjectured formula from the gravity side in the literature.
	
	The two main facets of AdS/CFT involve attempting to comprehend quantum gravity by utilizing superconformal field theories as a tool, and vice versa. In chapter \ref{ch:ads4log}, we use the bulk results to understand better the field theory results from supersymmetric localisation which are lack of explanation. In chapter \ref{ch:etheory}, we study the field theory using supersymmetric localisation to predict scattering amplitudes and the area of string worldsheet in supergravity. In chapter \ref{ch:ads8}, our main focus is in the bulk side and showed the absence of a phase transition, this encodes information of the strong coupling field theory dual.
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> chapters/manual/manual.tex <==
% !TeX root = ../../thesis.tex
\chapter{Manual}\label{ch:manual}


\section{Tips and Tricks}



\paragraph{Change cover font color:}
Add the command \texttt{\textbackslash color\{red\}} to the
\texttt{\textbackslash frontcoverheaderXII} command or enclose specific parts.
For example, \texttt{\{\textbackslash color\{red\}\textbackslash
textbf\{\textbackslash @authorf\textbackslash\ \textbackslash @authorl\}}.

\subsection{Full cover page}

\textbf{Important}: most printing services will create their own cover page based
on the details you send them (title, name, affiliation, ...) and do not supply
you with all necessary parameters (e.g., thickness of the paper) because these
differ from machine to machine. Therefore, the generated cover page is only
indicative and probably not used by your printing server (or even correct).


A full cover page (combining front cover, spine and back cover) can be
generated automatically using the command \texttt{make cover} or \texttt{python3 run.py cover}. This creates a pdf
\texttt{\$(COVERPDF);} by default this is \texttt{cover.pdf}.

The width of the spine is set by redefining \texttt{\\adsphdspinewidth} (9mm by default).

It can be seen in the provided \texttt{thesis.tex} that all information necessary to
generate a cover page is contained between two markers

\begin{verbatim}
    %%% COVER: Settings %%%
    ...
    %%% COVER: End settings %%%
\end{verbatim}

DO NOT REMOVE THESE!! They are used by the Makefile!!

The default front and/or back cover page can be overwritten: 

\begin{itemize}
    \item create a file \texttt{mycoverpage.tex}
    \item redefine the commands \texttt{\textbackslash makefrontcovergeneral} and \texttt{\textbackslash makebackcovergeneral}. For
          an example and more information, see the provided file \texttt{mycoverpage.tex}.
\end{itemize}

The cover page in the generated pdf has the following structure:

{\tiny
\begin{verbatim}
    <--rbleed--><--backcoverpage--><--lbleed--><--spine width--><--lbleed--><--frontcoverpage--><--rbleed-->
\end{verbatim}
}

The default bleed (both lbleed and rbleed) is 7mm. I suggest not changing this
value unless you know what you are doing ;) The latter can be done by
redefining \texttt{\textbackslash defaultlbleed} and \texttt{\textbackslash defaultrbleed} respectively.


\subsection{Table of contents}

To remove list of figures, tables and other preface chapters from the table of
contents, search for occurrences of \texttt{\textbackslash addcontentsline} in the file
\texttt{adsphd.cls} and comment them.

\subsection{Small ebook size}

When you add the \texttt{epub} option to the adsphd class the dissertation is
printed to a smaller size to read on a device such as Kindle.

Environments such as tables or tikZ pictures are often sized in absolute values
and not relative to the size of the output. You can wrap them in a resizebox
to enforce scaling:

\begin{verbatim}
  \resizebox{\textwidth}{!}{%
    \begin{tabular}{cc}
      ...
    \end{tabular}
  }
\end{verbatim}

\section{Settings for TeXstudio}

If you are working with TeXstudio or other windows latex editors you might want to adjust the editor's settings to allow a proper compilation of the table of contents and list of figures/tables.

\subsection{Custom \textit{makeindex} and \textit{makeglossaries} commands}

According to the \textit{README.md} the tables are indexed through two custom commands. To edit them in TeXstudio open the \textit{Commands} settings (\textit{Options $\to$ Configure TeXstudio...,  Commands} sheet), edit the following fields and press OK.

\textit{Makeindex}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.nlo -s nomencl.ist -o %.nls
\end{verbatim}}

\textit{Makeglossaries}:
{\scriptsize
\begin{verbatim}
"C:/Program Files/MiKTeX 2.9/miktex/bin/x64/makeindex.exe" %.glo -s %.ist -t %.glg -o %.gls
\end{verbatim}}

Now the customized commands can be launched by using \textit{Tools $\to$ Commands $\to$ MakeIndex/Makeglossaries}. If you want to automatize it in the standard \textit{Build \& View} (F5) and \textit{Compile} (F6) commands look at the following section.

\subsection{Custom Build\&View and Compile meta-commands}

Open \textit{Options $\to$ Configure TeXstudio...,  Build} sheet, edit the following field and press OK.

\textit{Build \& View}:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex
	\end{verbatim}}

To view the PDF once created you have to press F7 (or \textit{Tool $\to$ View}) and the PDF will automatically update in the default viewer whan you modify it. 

If you prefer to directly view the created PDF\textbf{ from the beginning }edit the field as follow:
{\footnotesize\begin{verbatim}
	txs:///pdflatex | txs:///bibtex | txs:///makeglossaries | txs:///makeindex |
	txs:///pdflatex  | txs:///pdflatex | txs:///view-pdf
	\end{verbatim}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage



==> chapters/preface/preface.tex <==
% !TeX root = ../../thesis.tex
\chapter*{Acknowledgements}                                  \label{ch:preface}

First and foremost, I would like to express my deepest gratitude to my supervisor, Nikolay, for his countless scientific instructions and encouragement in life. Your deep and sharp insights, reasonable criticism, sense of responsibility, and especially your diligence and enthusiasm for physics have greatly influenced me and taught me how a great physicist should be. Your eternal optimism and prompt jokes teach me to be confident and never to give up. You are always generous with your time and never mind sharing all of your knowledge and thoughts. Under your firm support and constant help, I gradually improved both my knowledge of physics and my life skills. How lucky I am to have been your student for the past five years! I can never repay your kindness, but I will forge ahead bravely and work hard in the future.

I would also like to thank my undergraduate supervisor, Bin Chen, for introducing me to our field and for all the useful advice and education. Thank you, M\'ark, for taking me as your student even when I didn't get the visa to meet you in person, and for your time guiding and teaching me.

I would like to thank the jury members, Tjonnie, Nikolay, Thomas H., Thomas v. R., Monica, and Christoph, for taking the time to carefully read my thesis and for all the valuable suggestions for improvement. Thank you, Annelien, for the help with the Dutch language.

This thesis would not have been possible without my brilliant collaborators: Nikolay, Pieter-Jan, Val, Junho, Marina, Pablo, Robert, Vasko, Angel, and Alberto. I have learned so much from collaborating and discussing with all of you. Pieter-Jan, you often come to my office with surprisingly new ideas and results, and you teach me how to run the codes hand-in-hand. All I know about Mathematica is largely attributed to you. Val, it has been a great pleasure working with you; I have learned so much from our discussions and am deeply impressed by your knowledge of math. Junho, you are always working so hard and keeping everything so organized, willing to help me with technical difficulties, and tolerating my unlimited procrastination (this point applies to all my collaborators). Marina, you are always full of energy and active in both work and life; it has been very enjoyable to be your collaborator and colleague. Thank you also for the jokes, which I know are from Reddit instead of from you. Pablo, I have always been amazed by your high efficiency in doing research. Thank you for carrying me through my first paper during graduate school, and also thanks for inviting me to the board games. Robert, we could have collaborated much more if it weren't for COVID, but I have benefited a lot from our work on 11d supergravity. Vasko, we could have interacted more without COVID as well. I enjoy our discussions and fun times both in physics and in real life.

The ITF is such a wonderful group with lovely people. Since 2019, I have spent four and a half years in this big family. I would like to start by thanking the ITF collectively for the fun times we have shared and the numerous discussions on physics. Special thanks to Anneleen for being so helpful and considerate, and for organizing everything so nicely. Thank you to the technicians, Filip, Bert, Jo, and Greg, for their help. I am grateful to all the faculty members for their attention and care: Toine, Joseph, Chris, Thomas H., Thomas v. R., Tjonnie, Wojciech, Daniel, Jonathan, and Bert V. Thanks to the research fellows at ITF for the enjoyable interactions and lots of help: Aidan, Anthony, Fotis, Israel, Brandon, Val, Pablo, Robert, Pieter-Jan, Junho, Jonas, Gianluca, Marina, Jo\~ao, Igal, Caroline, Hynek, Flavio, and Amir. I have also benefited a lot from the interactions with the ITF visitors: Sunjin, Alessandro P., Alfredo G. L., Ioannis L., Rishi, Pablo B., Noppadol, Shota, Tarek, Fri\dh rik, Dio, Gary, Dalimil, and Silviu. I am proud of being a graduate student here, among so many great peer students: Vincent M., Pieter B., Jesse, Lorenzo P., Kwinten, Nicol\`o Z., Rob, Vincent v. H., Vasko, Tijl, Sergio, Ludovico, Annelien, Joel, Faezeh, Oskar, Simon M., Simon K., S\'ebastien, Bruno, Gongrui, Milan, Arthur, Eva, Francesco C., Jihui, and Xiangwen. Thanks to the weekend club members, Faezeh, Sergio, Simon, Felipe, Bruno, Amir, Gongrui, and Thibaut, for making me less lonely during the weekends. Thanks to Sergio for voluntarily doing the dishwashing on weekends and evenings.

My visits to Saclay and SISSA have been very fruitful and enjoyable. Thank you to Val and Francesco for your warm hospitality, and to the institutes for their generosity. Thanks to Luca C., Ziming J., and Jesse for the happy time.

% The order: first the time-order of the conferences/schools. The joint Belgian seminars are in the beginning. For people appearing in multiple events, I assign them to the first event where we know each other. Within one event, if I know multiple people, I will sort according to my own personel preference based on the amount of interactions, the strength of our acquaintance. If there is no preference, I will sort according to the initial of FAMILY NAMES.

I would like to thank the organizers of all the academic events, conferences, and schools for their efforts in promoting knowledge and creating opportunities for people to interact, including giving me chances to present my own work. Special thanks to the organizers of the Belgian joint hep-th seminars, the Solvay Doctoral School, the Carg\`ese School, the CERN Winter School, EuroStrings, Strings, Supergravity, and the ICTP Workshop for their great work. Maria, Dongming, Seppe, Gabriel L., Pietro B. G., Yan L., Jani, Yixuan, Peng C., Jiaxin, Yi Z., Deliang, Ziming J., Kaiwen, Zhizhen, Chris H., Shuwei, Lecheng, Xin W., Zhuoyu, Xuyao, Zhaohui, Yangrui, Bogdan, Anthony H., Davide C., Alejandro C., Nejc, Bin Z., Sonja, Guanhao, Xiaoyue, Tian T., Huiyu, Tianli, Aaron, Loc, Cynthia, Minsung, Yoda, Shing Yan, Gordon L., Muthu, Rohit, Michelle, Yorgo, Jan, Christian J., Dan, Stathis, Gabriele, Aike, Mart\'i, Michele, Ayngaran, Sunandan, Wei F., Vineeth, Ana, Silvia, Victor, Ohad, Tom\'as, and so many others, I feel very happy to have met all of you.

Applying for post-doc positions has been a tough time. I would like to thank my recommenders, Nikolay, Thomas, Val, and Junho, for doing me this great favor and for their help with my application documents. Thank you, Hossein, Hao Z., Jun, and Cheng P., for kindly introducing the group. Thank you, Nikolay, Val, Bin C., Jia T., Zhefei, Luca C., Vincent v. H., Kaiwen, Han L., Ziruo, and Yuan Z., for the valuable advice.

My most special thanks go to my girlfriend, Xiaohong. Despite being thousands of miles away, she always brings me so much happiness and fulfillment. I cannot help but look forward to the life we will share together in the future. Thanks to my mom and dad for their unwavering support and encouragement. It means a lot to me. 

% Ordering: relationship order > time order.

Ninety percent of my time has been spent in my apartment and the office, so I would like to thank my roommates and office mates, Zhenyu Z., Chao J., Heng C., Zhenhong, Hao L., Xueliang, Xuan Z., Haoying C., Wei G., Felipe, Amir, Tijl, Thibaut, and Bram, for their care, tolerance, and joy. I feel very lucky to be a member of the ``Family of LSP'' and the office 06.01. Thanks also to my Chinese friends Zhaolei, Yang L., Jiawei H., Yong L., Zhongwu, Sijie, Wei Z., Hui P., Hongwei, Zhongchen, Juntong, Bingxin, Ning H., and those already mentioned above, for the support and fun times.

I would like to thank all of my friends not already mentioned above; thank you for the fun times we spent together. It is amazing that our worldlines crossed in the immense ranges of space and time of the universe.

The first two years of my time in Leuven were under the shadow of the COVID-19 pandemic. It was painful for everyone, both physically and mentally.\footnote{For example, there was always a mask on my face until the beginning of 2023, which is only one and a half years ago.} I would like to sincerely thank all the medical workers for their great sacrifices and efforts in fighting against the pandemic; you are truly the heroes of humanity. The seemingly small efforts made by everyone in their daily lives are also highly valuable and appreciated.

People say that doing a Ph.D. is like a lonely journey. During the long process, there has been loneliness, difficulty, confusion, sorrow, regret, fear, hesitation, anxiety, and frustration. It is because of all of you that this journey has also been filled with company, hope, enlightenment, happiness, comfort, bravery, faith, serenity, and encouragement. I wish that time could slow down a bit so that I can enjoy this moment of life, but the sun is setting. If I have to say goodbye to some of you, I hope our future will be bright.

\begin{flushright}
	Xuao Zhang, Leuven, July 2024
\end{flushright}

% \instructionspreface


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> mycoverpage.tex <==
% Redefine in this file the commands to generate the front and back cover:
%
%   \makefrontcovergeneral{xskip}{clearpage}
%   \makebackcovergeneral{xskip}{clearpage}
%
% You can start from their definition in adsphd.cls. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% My own cover page
\makeatletter

%% \renewcommand{\makefrontcovergeneral}[2]{%
%%   %
%%   % Create header
%%   \frontcoverheader{#1}
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Title, subtitle, authorname, text and date can be moved around.
%%   % Change the textblock* commands below. 
%%   %
%%   % Syntax of textblock environment:
%%   % 
%%   %   \begin{textblock*}{width}(xpos,ypos)
%%   %     ...
%%   %   \end{textblock*}
%%   % 
%%   % !! Make sure not to remove the '+#1' part!!!
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Place the title
%%   \begin{textblock*}{120mm}(17.5mm+#1,89.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \raggedright\selectfont\LARGE\sffamily\textbf{\@title}
%%   \end{textblock*}
%%   %
%%   % Place the subtitle
%%   \begin{textblock*}{120mm}(17.5mm+#1,92.0mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily{\@subtitle}
%%   \end{textblock*}
%%   %
%%   % Place the author name
%%   \begin{textblock*}{120mm}(17.5mm+#1,109.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \Large\sffamily\@authorf\ \MakeUppercase\@authorl
%%   \end{textblock*}
%%   %
%%   %\begin{textblock}{120}(0,115)
%%   \begin{textblock*}{120mm}(17.5mm+#1,132.0mm)
%%   \textblockcolour{}
%%   \includegraphics*{image/coverfigure}
%%   \end{textblock*}
%%   %
%%   % Place the misc text
%%   \begin{textblock*}{60mm}(96.5mm+#1,187.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   {\small\sffamily Dissertation presented in partial\\
%%   fulfillment of the requirements for\\
%%   the degree of Doctor\\
%%   in \@degree}
%%   \end{textblock*}
%%   %
%%   % Place date
%%   \begin{textblock*}{160mm}(0mm+#1,221.5mm)
%%   \textblockcolour{}
%%   \vspace{-\parskip}
%%   \begin{center} {\small\sffamily\@date }\end{center}
%%   \end{textblock*}
%%   
%%   %
%%   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%   %
%%   % Add footer
%%   \frontcoverfooter{#2}
%% 
%% }

\makeatother

